A soft nearest-neighbor framework for continual semi-supervised learning

Despite significant advances, the performance of state-of-the-art continual learning approaches hinges on the unrealistic scenario of fully labeled data. In this paper, we tackle this challenge and propose an approach for continual semi-supervised learning--a setting where not all the data samples are labeled. A primary issue in this scenario is the model forgetting representations of unlabeled data and overfitting the labeled samples. We leverage the power of nearest-neighbor classifiers to nonlinearly partition the feature space and flexibly model the underlying data distribution thanks to its non-parametric nature. This enables the model to learn a strong representation for the current task, and distill relevant information from previous tasks. We perform a thorough experimental evaluation and show that our method outperforms all the existing approaches by large margins, setting a solid state of the art on the continual semi-supervised learning paradigm. For example, on CIFAR-100 we surpass several others even when using at least 30 times less supervision (0.8% vs. 25% of annotations). Finally, our method works well on both low and high resolution images and scales seamlessly to more complex datasets such as ImageNet-100. The code is publicly available on https://github.com/kangzhiq/NNCSL

==> egbib_old.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@inproceedings{assran2021semi,
  title={Semi-supervised learning of visual features by non-parametrically predicting view assignments with support samples},
  author={Assran, Mahmoud and Caron, Mathilde and Misra, Ishan and Bojanowski, Piotr and Joulin, Armand and Ballas, Nicolas and Rabbat, Michael},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={8443--8452},
  year={2021}
}


@inproceedings{wang2021ordisco,
  title={Ordisco: Effective and efficient usage of incremental unlabeled data for semi-supervised continual learning},
  author={Wang, Liyuan and Yang, Kuo and Li, Chongxuan and Hong, Lanqing and Li, Zhenguo and Zhu, Jun},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5383--5392},
  year={2021}
}

@article{boschini2022continual,
  title={Continual semi-supervised learning through contrastive interpolation consistency},
  author={Boschini, Matteo and Buzzega, Pietro and Bonicelli, Lorenzo and Porrello, Angelo and Calderara, Simone},
  journal={Pattern Recognition Letters},
  volume={162},
  pages={9--14},
  year={2022},
  publisher={Elsevier}
}

@article{de2021continual,
  title={A continual learning survey: Defying forgetting in classification tasks},
  author={De Lange, Matthias and Aljundi, Rahaf and Masana, Marc and Parisot, Sarah and Jia, Xu and Leonardis, Ale{\v{s}} and Slabaugh, Gregory and Tuytelaars, Tinne},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={44},
  number={7},
  pages={3366--3385},
  year={2021}
}

@inproceedings{zhai2019s4l,
  title={S4l: Self-supervised semi-supervised learning},
  author={Zhai, Xiaohua and Oliver, Avital and Kolesnikov, Alexander and Beyer, Lucas},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1476--1485},
  year={2019}
}

@article{chen2022debiased,
  title={Debiased Pseudo Labeling in Self-Training},
  author={Chen, Baixu and Jiang, Junguang and Wang, Ximei and Wang, Jianmin and Long, Mingsheng},
  journal={arXiv preprint arXiv:2202.07136},
  year={2022}
}

@article{sohn2020fixmatch,
  title={Fixmatch: Simplifying semi-supervised learning with consistency and confidence},
  author={Sohn, Kihyuk and Berthelot, David and Carlini, Nicholas and Zhang, Zizhao and Zhang, Han and Raffel, Colin A and Cubuk, Ekin Dogus and Kurakin, Alexey and Li, Chun-Liang},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={596--608},
  year={2020}
}

@inproceedings{lee2013pseudo,
  title={Pseudo-label: The simple and efficient semi-supervised learning method for deep neural networks},
  author={Lee, Dong-Hyun and others},
  booktitle={Workshop on challenges in representation learning, ICML},
  volume={3},
  number={2},
  pages={896},
  year={2013}
}

@article{li2018pami,
author={Li, Zhizhong and Hoiem, Derek},
title={Learning Without Forgetting},
journal={Trans.\ PAMI},
year="2018",
}

@inproceedings{rebuffi2017cvpr,
  title={{iCaRL}: Incremental Classifier and Representation Learning},
  author={Sylvestre-Alvise Rebuffi and Alexander Kolesnikov and Georg Sperl and Christoph H. Lampert},
  booktitle={CVPR},
  year={2017}
}

@InProceedings{prabhu20,
author="Prabhu, Ameya
and Torr, Philip H. S.
and Dokania, Puneet K.",
title="GDumb: A Simple Approach that Questions Our Progress in Continual Learning",
booktitle="ECCV",
year="2020",
npages="524--540",
}

% % review
@article{chen2022semi,
  title={Semi-Supervised and Unsupervised Deep Visual Learning: A Survey},
  author={Chen, Yanbei and Mancini, Massimiliano and Zhu, Xiatian and Akata, Zeynep},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2022},
  publisher={IEEE}
}

%%%% consistency regularization models

%% consistency over model perturbation
@article{sajjadi2016regularization,
  title={Regularization with stochastic transformations and perturbations for deep semi-supervised learning},
  author={Sajjadi, Mehdi and Javanmardi, Mehran and Tasdizen, Tolga},
  journal={Advances in neural information processing systems},
  volume={29},
  year={2016}
}

@inproceedings{laine2017temporal,
  title={Temporal Ensembling for Semi-Supervised Learning},
  author={Samuli Laine and Timo Aila},
  booktitle={International Conference on Learning Representations},
  year={2017},
}

@inproceedings{miyato2016distributional,
  title={Distributional smoothing with virtual adversarial training},
  author={Miyato, Takeru and Maeda, Shin-ichi and Koyama, Masanori and Nakae, Ken and Ishii, Shin},
  booktitle={International Conference on Learning Representations},
  year={2016}
}


@inproceedings{park2018adversarial,
  title={Adversarial dropout for supervised and semi-supervised learning},
  author={Park, Sungrae and Park, JunKeon and Shin, Su-Jin and Moon, Il-Chul},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={32},
  number={1},
  year={2018}
}

@article{tarvainen2017mean,
  title={Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
  author={Tarvainen, Antti and Valpola, Harri},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{athiwaratkun2019there,
  title={There are many consistent explanations of unlabeled data: Why you should average},
  author={Athiwaratkun, Ben and Finzi, Marc and Izmailov, Pavel and Wilson, Andrew Gordon},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{zhang2020wcp,
  title={Wcp: Worst-case perturbations for semi-supervised deep learning},
  author={Zhang, Liheng and Qi, Guo-Jun},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3912--3921},
  year={2020}
}

%%%% pseudo-labelling

@inproceedings{lee2013pseudo,
  title={Pseudo-label: The simple and efficient semi-supervised learning method for deep neural networks},
  author={Lee, Dong-Hyun and others},
  booktitle={Workshop on challenges in representation learning, ICML},
  volume={3},
  number={2},
  pages={896},
  year={2013}
}

@inproceedings{arazo2020pseudo,
  title={Pseudo-labeling and confirmation bias in deep semi-supervised learning},
  author={Arazo, Eric and Ortego, Diego and Albert, Paul and O’Connor, Noel E and McGuinness, Kevin},
  booktitle={International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}


@inproceedings{xie2020self,
  title={Self-training with noisy student improves imagenet classification},
  author={Xie, Qizhe and Luong, Minh-Thang and Hovy, Eduard and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={10687--10698},
  year={2020}
}

%% debaised

@article{chen2022debiased,
  title={Debiased Pseudo Labeling in Self-Training},
  author={Chen, Baixu and Jiang, Junguang and Wang, Ximei and Wang, Jianmin and Long, Mingsheng},
  journal={arXiv preprint arXiv:2202.07136},
  year={2022}
}

% another debiased pseudo-labeling method (rejected eccv22)
@article{schmutz2022don,
  title={Don't fear the unlabelled: safe deep semi-supervised learning via simple debiaising},
  author={Schmutz, Hugo and Humbert, Olivier and Mattei, Pierre-Alexandre},
  journal={arXiv preprint arXiv:2203.07512},
  year={2022}
}

@inproceedings{wang2022debiased,
  title={Debiased Learning from Naturally Imbalanced Pseudo-Labels},
  author={Wang, Xudong and Wu, Zhirong and Lian, Long and Yu, Stella X},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14647--14657},
  year={2022}
}

%%%% hybrid

%% student teacher
@article{sohn2020fixmatch,
  title={Fixmatch: Simplifying semi-supervised learning with consistency and confidence},
  author={Sohn, Kihyuk and Berthelot, David and Carlini, Nicholas and Zhang, Zizhao and Zhang, Han and Raffel, Colin A and Cubuk, Ekin Dogus and Kurakin, Alexey and Li, Chun-Liang},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={596--608},
  year={2020}
}

%% with smarter thresholding
@inproceedings{li2021comatch,
  title={Comatch: Semi-supervised learning with contrastive graph regularization},
  author={Li, Junnan and Xiong, Caiming and Hoi, Steven CH},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9475--9484},
  year={2021}
}


@article{zhang2021flexmatch,
  title={Flexmatch: Boosting semi-supervised learning with curriculum pseudo labeling},
  author={Zhang, Bowen and Wang, Yidong and Hou, Wenxin and Wu, Hao and Wang, Jindong and Okumura, Manabu and Shinozaki, Takahiro},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={18408--18419},
  year={2021}
}

@inproceedings{xu2021dash,
  title={Dash: Semi-supervised learning with dynamic thresholding},
  author={Xu, Yi and Shang, Lei and Ye, Jinxing and Qian, Qi and Li, Yu-Feng and Sun, Baigui and Li, Hao and Jin, Rong},
  booktitle={International Conference on Machine Learning},
  pages={11525--11536},
  year={2021},
  organization={PMLR}
}

@inproceedings{pham2021meta,
  title={Meta pseudo labels},
  author={Pham, Hieu and Dai, Zihang and Xie, Qizhe and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11557--11568},
  year={2021}
}

%% uncertainty

@inproceedings{chen2020semi,
  title={Semi-supervised learning under class distribution mismatch},
  author={Chen, Yanbei and Zhu, Xiatian and Li, Wei and Gong, Shaogang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={04},
  pages={3569--3576},
  year={2020}
}

@inproceedings{rizve2021defense,
  title={In defense of pseudo-labeling: An uncertainty-aware pseudo-label selection framework for semi-supervised learning},
  author={Rizve, Mamshad Nayeem and Duarte, Kevin and Rawat, Yogesh S and Shah, Mubarak},
  booktitle={International Conference on Learning Representations},
  year={2021}
}

@inproceedings{wang2022np,
  title={Np-match: When neural processes meet semi-supervised learning},
  author={Wang, Jianfeng and Lukasiewicz, Thomas and Massiceti, Daniela and Hu, Xiaolin and Pavlovic, Vladimir and Neophytou, Alexandros},
  booktitle={International Conference on Machine Learning},
  pages={22919--22934},
  year={2022},
  organization={PMLR}
}

%% mixup based

@inproceedings{verma2019interpolation,
  title={Interpolation consistency training for semi-supervised learning},
  author={Verma, Vikas and Kawaguchi, Kenji and Lamb, Alex and Kannala, Juho and Bengio, Yoshua and Lopez-Paz, David},
  booktitle={Proceedings of the International Joint Conference on Artificial Intelligence, {IJCAI}},
  pages={3635--3641},
  year={2019}
}

@article{berthelot2019mixmatch,
  title={Mixmatch: A holistic approach to semi-supervised learning},
  author={Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin A},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{berthelot2020remixmatch,
  title={Remixmatch: Semi-supervised learning with distribution alignment and augmentation anchoring},
  author={Berthelot, David and Carlini, Nicholas and Cubuk, Ekin D and Kurakin, Alex and Sohn, Kihyuk and Zhang, Han and Raffel, Colin},
  booktitle={International Conference on Learning Representations},
  year={2020}
}

@article{liu2022decoupled,
  title={Decoupled Mixup for Data-efficient Learning},
  author={Liu, Zicheng and Li, Siyuan and Wang, Ge and Tan, Cheng and Wu, Lirong and Li, Stan Z},
  journal={arXiv preprint arXiv:2203.10761},
  year={2022}
}

@inproceedings{da2022dual,
  title={Dual-Head Contrastive Domain Adaptation for Video Action Recognition},
  author={da Costa, Victor G Turrisi and Zara, Giacomo and Rota, Paolo and Oliveira-Santos, Thiago and Sebe, Nicu and Murino, Vittorio and Ricci, Elisa},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={1181--1190},
  year={2022}
}

@article{jaiswal2020survey,
  title={A survey on contrastive self-supervised learning},
  author={Jaiswal, Ashish and Babu, Ashwin Ramesh and Zadeh, Mohammad Zaki and Banerjee, Debapriya and Makedon, Fillia},
  journal={Technologies},
  volume={9},
  number={1},
  pages={2},
  year={2020},
  publisher={MDPI}
}

%% augmentation based
@article{xie2020unsupervised,
  title={Unsupervised data augmentation for consistency training},
  author={Xie, Qizhe and Dai, Zihang and Hovy, Eduard and Luong, Thang and Le, Quoc},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={6256--6268},
  year={2020}
}

@inproceedings{zheng2022simmatch,
  title={SimMatch: Semi-supervised Learning with Similarity Matching},
  author={Zheng, Mingkai and You, Shan and Huang, Lang and Wang, Fei and Qian, Chen and Xu, Chang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14471--14481},
  year={2022}
}

@inproceedings{kim2022conmatch,
  title={ConMatch: Semi-Supervised Learning with Confidence-Guided Consistency Regularization},
  author={Kim, Jiwon and Min, Youngjo and Kim, Daehwan and Lee, Gyuseong and Seo, Junyoung and Ryoo, Kwangrok and Kim, Seungryong},
  booktitle={European Conference on Computer Vision},
  year={2022}
}
 %%%% co-trainining

@inproceedings{qiao2018deep,
  title={Deep co-training for semi-supervised image recognition},
  author={Qiao, Siyuan and Shen, Wei and Zhang, Zhishuai and Wang, Bo and Yuille, Alan},
  booktitle={Proceedings of the european conference on computer vision (eccv)},
  pages={135--152},
  year={2018}
}

@inproceedings{dong2018tri,
  title={Tri-net for semi-supervised deep learning},
  author={Dong-DongChen, WeiWang and WeiGao, Zhi-HuaZhou},
  booktitle={Proceedings of twenty-seventh international joint conference on artificial intelligence},
  pages={2014--2020},
  year={2018}
}



%%%% SSL-inspired

@article{wang2020enaet,
  title={EnAET: A self-trained framework for semi-supervised and supervised learning with ensemble transformations},
  author={Wang, Xiao and Kihara, Daisuke and Luo, Jiebo and Qi, Guo-Jun},
  journal={IEEE Transactions on Image Processing},
  volume={30},
  pages={1639--1647},
  year={2020},
  publisher={IEEE}
}

@inproceedings{zhai2019s4l,
  title={S4l: Self-supervised semi-supervised learning},
  author={Zhai, Xiaohua and Oliver, Avital and Kolesnikov, Alexander and Beyer, Lucas},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1476--1485},
  year={2019}
}

@article{chen2020big,
  title={Big self-supervised models are strong semi-supervised learners},
  author={Chen, Ting and Kornblith, Simon and Swersky, Kevin and Norouzi, Mohammad and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={22243--22255},
  year={2020}
}

@article{assran2020supervision,
  title={Supervision accelerates pre-training in contrastive semi-supervised learning of visual representations},
  author={Assran, Mahmoud and Ballas, Nicolas and Castrejon, Lluis and Rabbat, Michael},
  journal={arXiv preprint arXiv:2006.10803},
  year={2020}
}

@inproceedings{assran2021semi,
  title={Semi-supervised learning of visual features by non-parametrically predicting view assignments with support samples},
  author={Assran, Mahmoud and Caron, Mathilde and Misra, Ishan and Bojanowski, Piotr and Joulin, Armand and Ballas, Nicolas and Rabbat, Michael},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={8443--8452},
  year={2021}
}

@inproceedings{assran2022masked,
  title={Masked siamese networks for label-efficient learning},
  author={Assran, Mahmoud and Caron, Mathilde and Misra, Ishan and Bojanowski, Piotr and Bordes, Florian and Vincent, Pascal and Joulin, Armand and Rabbat, Mike and Ballas, Nicolas},
  booktitle={European Conference on Computer Vision},
  pages={456--473},
  year={2022},
  organization={Springer}
}

@inproceedings{lucas2022barely,
  title={Barely-supervised learning: semi-supervised learning with very few labeled images},
  author={Lucas, Thomas and Weinzaepfel, Philippe and Rogez, Gregory},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={36},
  number={2},
  pages={1881--1889},
  year={2022}
}

@inproceedings{cai2021exponential,
  title={Exponential moving average normalization for self-supervised and semi-supervised learning},
  author={Cai, Zhaowei and Ravichandran, Avinash and Maji, Subhransu and Fowlkes, Charless and Tu, Zhuowen and Soatto, Stefano},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={194--203},
  year={2021}
}

@article{kim2021selfmatch,
  title={Selfmatch: Combining contrastive self-supervision and consistency for semi-supervised learning},
  author={Kim, Byoungjip and Choo, Jinho and Kwon, Yeong-Dae and Joe, Seongho and Min, Seungjai and Gwon, Youngjune},
  journal={arXiv preprint arXiv:2101.06480},
  year={2021}
}

%%%%
%%%% clustering-based models
%%%%

@inproceedings{asano2020self,
  title={Self-labelling via simultaneous clustering and representation learning},
  author={Asano, Yuki Markus and Rupprecht, Christian and Vedaldi, Andrea},
  booktitle={International Conference on Learning Representations},
  year={2020}
}

@inproceedings{li2021prototypical,
  title={Prototypical Contrastive Learning of Unsupervised Representations},
  author={Junnan Li and Pan Zhou and Caiming Xiong and Steven Hoi},
  booktitle={International Conference on Learning Representations},
  year={2021}
}

@inproceedings{caron2018deep,
  title={Deep clustering for unsupervised learning of visual features},
  author={Caron, Mathilde and Bojanowski, Piotr and Joulin, Armand and Douze, Matthijs},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={132--149},
  year={2018}
}

@article{caron2020unsupervised,
  title={Unsupervised learning of visual features by contrasting cluster assignments},
  author={Caron, Mathilde and Misra, Ishan and Mairal, Julien and Goyal, Priya and Bojanowski, Piotr and Joulin, Armand},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={9912--9924},
  year={2020}
}

@inproceedings{caron2021emerging,
  title={Emerging properties in self-supervised vision transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J{\'e}gou, Herv{\'e} and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9650--9660},
  year={2021}
}

%%%%
%%%% selfsup literature
%%%%

@inproceedings{he2022masked,
  title={Masked autoencoders are scalable vision learners},
  author={He, Kaiming and Chen, Xinlei and Xie, Saining and Li, Yanghao and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={16000--16009},
  year={2022}
}

@article{vincent2010stacked,
  title={Stacked denoising autoencoders: Learning useful representations in a deep network with a local denoising criterion.},
  author={Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine and Bottou, L{\'e}on},
  journal={Journal of machine learning research},
  volume={11},
  number={12},
  year={2010}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}

@article{chen2020improved,
  title={Improved baselines with momentum contrastive learning},
  author={Chen, Xinlei and Fan, Haoqi and Girshick, Ross and He, Kaiming},
  journal={arXiv preprint arXiv:2003.04297},
  year={2020}
}

@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={9729--9738},
  year={2020}
}

@inproceedings{mitrovic2021representation,
  title={Representation Learning via Invariant Causal Mechanisms},
  author={Mitrovic, Jovana and McWilliams, Brian and Walker, Jacob and Buesing, Lars and Blundell, Charles},
  booktitle={International Conference on Learning Representations},
  year={2021},
}

@article{bachman2019learning,
  title={Learning representations by maximizing mutual information across views},
  author={Bachman, Philip and Hjelm, R Devon and Buchwalter, William},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@article{grill2020bootstrap,
  title={Bootstrap your own latent-a new approach to self-supervised learning},
  author={Grill, Jean-Bastien and Strub, Florian and Altch{\'e}, Florent and Tallec, Corentin and Richemond, Pierre and Buchatskaya, Elena and Doersch, Carl and Avila Pires, Bernardo and Guo, Zhaohan and Gheshlaghi Azar, Mohammad and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21271--21284},
  year={2020}
}

@inproceedings{wu2018unsupervised,
  title={Unsupervised feature learning via non-parametric instance discrimination},
  author={Wu, Zhirong and Xiong, Yuanjun and Yu, Stella X and Lin, Dahua},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3733--3742},
  year={2018}
}

@article{oord2018representation,
  title={Representation learning with contrastive predictive coding},
  author={Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1807.03748},
  year={2018}
}

@inproceedings{gutmann2010noise,
  title={Noise-contrastive estimation: A new estimation principle for unnormalized statistical models},
  author={Gutmann, Michael and Hyv{\"a}rinen, Aapo},
  booktitle={Proceedings of the thirteenth international conference on artificial intelligence and statistics},
  pages={297--304},
  year={2010},
  organization={JMLR Workshop and Conference Proceedings}
}

@inproceedings{chen2021exploring,
  title={Exploring simple siamese representation learning},
  author={Chen, Xinlei and He, Kaiming},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15750--15758},
  year={2021}
}

@inproceedings{zbontar2021barlow,
  title={Barlow twins: Self-supervised learning via redundancy reduction},
  author={Zbontar, Jure and Jing, Li and Misra, Ishan and LeCun, Yann and Deny, St{\'e}phane},
  booktitle={International Conference on Machine Learning},
  pages={12310--12320},
  year={2021},
  organization={PMLR}
}

@inproceedings{bardes2022vicreg,
  title={{VICR}eg: Variance-Invariance-Covariance Regularization for Self-Supervised Learning},
  author={Bardes, Adrien and Ponce, Jean and LeCun, Yann},
  booktitle={International Conference on Learning Representations},
  year={2022},
}

@inproceedings{bardes2022vicregl,
  author  = {Adrien Bardes and Jean Ponce and Yann LeCun},
  title   = {VICRegL: Self-Supervised Learning of Local Visual Features},
  booktitle = {NeurIPS},
  year    = {2022},
}

@inproceedings{ermolov2021whitening,
  title={Whitening for self-supervised representation learning},
  author={Ermolov, Aleksandr and Siarohin, Aliaksandr and Sangineto, Enver and Sebe, Nicu},
  booktitle={International Conference on Machine Learning},
  pages={3015--3024},
  year={2021},
  organization={PMLR}
}



@article{rao2019continual,
  title={Continual unsupervised representation learning},
  author={Rao, Dushyant and Visin, Francesco and Rusu, Andrei A and Teh, Yee Whye and Pascanu, Razvan and Hadsell, Raia},
  journal=NIPS,
  year={2019}
}

@article{smith2019unsupervised,
  title={Unsupervised progressive learning and the stam architecture},
  author={Smith, James and Taylor, Cameron and Baer, Seth and Dovrolis, Constantine},
  journal={arXiv preprint arXiv:1904.02021},
  year={2019}
}

@article{achille2018life,
  title={Life-long disentangled representation learning with cross-domain latent homologies},
  author={Achille, Alessandro and Eccles, Tom and Matthey, Loic and Burgess, Christopher P and Watters, Nick and Lerchner, Alexander and Higgins, Irina},
  journal=NIPS,
  year={2018}
}

@article{gallardo2021self,
  title={Self-Supervised Training Enhances Online Continual Learning},
  author={Gallardo, Jhair and Hayes, Tyler L and Kanan, Christopher},
  journal={arXiv preprint arXiv:2103.14010},
  year={2021}
}

@article{caccia2021special,
  title={SPeCiaL: Self-Supervised Pretraining for Continual Learning},
  author={Caccia, Lucas and Pineau, Joelle},
  journal={arXiv preprint arXiv:2106.09065},
  year={2021}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={ICML},
  year={2020},
}

@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle=CVPR,
  year={2020}
}

@article{zbontar2021barlow,
  title={Barlow twins: Self-supervised learning via redundancy reduction},
  author={Zbontar, Jure and Jing, Li and Misra, Ishan and LeCun, Yann and Deny, St{\'e}phane},
  journal={ICML},
  year={2021}
}

@article{bardes2021vicreg,
  title={Vicreg: Variance-invariance-covariance regularization for self-supervised learning},
  author={Bardes, Adrien and Ponce, Jean and LeCun, Yann},
  journal={arXiv preprint arXiv:2105.04906},
  year={2021}
}

@inproceedings{ermolov2021whitening,
  title={Whitening for self-supervised representation learning},
  author={Ermolov, Aleksandr and Siarohin, Aliaksandr and Sangineto, Enver and Sebe, Nicu},
  booktitle={ICML},
  year={2021},
}

@article{caron2020unsupervised,
  title={Unsupervised learning of visual features by contrasting cluster assignments},
  author={Caron, Mathilde and Misra, Ishan and Mairal, Julien and Goyal, Priya and Bojanowski, Piotr and Joulin, Armand},
  journal=NIPS,
  year={2020}
}

@article{caron2021emerging,
  title={Emerging properties in self-supervised vision transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J{\'e}gou, Herv{\'e} and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  journal=ICCV,
  year={2021}
}

@article{grill2020bootstrap,
  title={Bootstrap your own latent: A new approach to self-supervised learning},
  author={Grill, Jean-Bastien and Strub, Florian and Altch{\'e}, Florent and Tallec, Corentin and Richemond, Pierre H and Buchatskaya, Elena and Doersch, Carl and Pires, Bernardo Avila and Guo, Zhaohan Daniel and Azar, Mohammad Gheshlaghi and others},
  journal=NIPS,
  year={2020}
}

@inproceedings{chen2021exploring,
  title={Exploring simple siamese representation learning},
  author={Chen, Xinlei and He, Kaiming},
  booktitle=ICCV,
  year={2021}
}

@article{dwibedi2021little,
  title={With a little help from my friends: Nearest-neighbor contrastive learning of visual representations},
  author={Dwibedi, Debidatta and Aytar, Yusuf and Tompson, Jonathan and Sermanet, Pierre and Zisserman, Andrew},
  journal=ICCV,
  year={2021}
}


@article{turrisi2021sololearn,
      title={Solo-learn: A Library of Self-supervised Methods for Visual Representation Learning}, 
      author={Victor G. Turrisi da Costa and Enrico Fini and Moin Nabi and Nicu Sebe and Elisa Ricci},
      year={2021},
      journal={arXiv 2108.01775},
      eprint={2108.01775},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={\url{https://github.com/vturrisi/solo-learn}},
}

@inproceedings{hou2019learning,
  title={Learning a unified classifier incrementally via rebalancing},
  author={Hou, Saihui and Pan, Xinyu and Loy, Chen Change and Wang, Zilei and Lin, Dahua},
  booktitle=CVPR,
  pages={831--839},
  year={2019}
}

@inproceedings{wang2019pay,
  title={Pay attention to features, transfer learn faster CNNs},
  author={Wang, Kafeng and Gao, Xitong and Zhao, Yiren and Li, Xingjian and Dou, Dejing and Xu, Cheng-Zhong},
  booktitle=ICLR,
  year={2019}
}

@inproceedings{komodakis2017paying,
  title={Paying more attention to attention: improving the performance of convolutional neural networks via attention transfer},
  author={Komodakis, Nikos and Zagoruyko, Sergey},
  booktitle=ICLR,
  year={2017}
}

@inproceedings{dhar2019learning,
  title={Learning without memorizing},
  author={Dhar, Prithviraj and Singh, Rajat Vikram and Peng, Kuan-Chuan and Wu, Ziyan and Chellappa, Rama},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{douillard2020podnet,
  title={Podnet: Pooled outputs distillation for small-tasks incremental learning},
  author={Douillard, Arthur and Cord, Matthieu and Ollion, Charles and Robert, Thomas and Valle, Eduardo},
  booktitle=ECCV,
  year={2020},
}

@article{liu2020continual,
  title={Continual universal object detection},
  author={Liu, Xialei and Yang, Hao and Ravichandran, Avinash and Bhotika, Rahul and Soatto, Stefano},
  journal={arXiv preprint arXiv:2002.05347},
  year={2020}
}

@article{lin2021continual,
  title={Continual Contrastive Self-supervised Learning for Image Classification},
  author={Lin, Zhiwei and Wang, Yongtao and Lin, Hongxiang},
  journal={arXiv preprint arXiv:2107.01776},
  year={2021}
}


@article{madaan2021rethinking,
  title={Rethinking the Representational Continuity: Towards Unsupervised Continual Learning},
  author={Madaan, Divyam and Yoon, Jaehong and Li, Yuanchun and Liu, Yunxin and Hwang, Sung Ju},
  journal={arXiv preprint arXiv:2110.06976},
  year={2021}
}

@inproceedings{caron2018deep,
  title={Deep clustering for unsupervised learning of visual features},
  author={Caron, Mathilde and Bojanowski, Piotr and Joulin, Armand and Douze, Matthijs},
  booktitle=ECCV,
  pages={132--149},
  year={2018}
}

@inproceedings{caron2019unsupervised,
  title={Unsupervised pre-training of image features on non-curated data},
  author={Caron, Mathilde and Bojanowski, Piotr and Mairal, Julien and Joulin, Armand},
  booktitle=ICCV,
  pages={2959--2968},
  year={2019}
}

@article{chen2020improved,
  title={Improved baselines with momentum contrastive learning},
  author={Chen, Xinlei and Fan, Haoqi and Girshick, Ross and He, Kaiming},
  journal={arXiv preprint arXiv:2003.04297},
  year={2020}
}

@article{khosla2020supervised,
  title={Supervised contrastive learning},
  author={Khosla, Prannay and Teterwak, Piotr and Wang, Chen and Sarna, Aaron and Tian, Yonglong and Isola, Phillip and Maschinot, Aaron and Liu, Ce and Krishnan, Dilip},
  journal=NIPS,
  year={2020}
}

@article{de2019continual,
  title={Continual learning: A comparative study on how to defy forgetting in classification tasks},
  author={De Lange, Matthias and Aljundi, Rahaf and Masana, Marc and Parisot, Sarah and Jia, Xu and Leonardis, Ales and Slabaugh, Gregory and Tuytelaars, Tinne},
  journal=PAMI,
  volume={2},
  number={6},
  year={2019}
}

@article{French99,
author={French, Robert M.},
doi={10.1016/S1364-6613(99)01294-2},
isbn={13646613},
issn={13646613},
journal={Trends in Cognitive Sciences},
number={4},
pages={128--135},
pmid={10322466},
title={Catastrophic forgetting in connectionist networks},
volume={3},
year={1999},
keywords={Classic},
url={https://www.sciencedirect.com/science/article/abs/pii/S1364661399012942}
}

@inproceedings{Mccloskey89,
  title={Catastrophic interference in connectionist networks: The sequential learning problem},
  author={McCloskey, Michael and Cohen, Neal J},
  booktitle={Psychology of learning and motivation},
  volume={24},
  pages={109--165},
  year={1989},
  publisher={Elsevier},
  keywords={Classics},
  url={https://www.sciencedirect.com/science/article/pii/S0079742108605368}
}

@article{mikolov2013efficient,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={NAACL},
  year={2018}
}

@inproceedings{wu2018unsupervised,
  title={Unsupervised feature learning via non-parametric instance discrimination},
  author={Wu, Zhirong and Xiong, Yuanjun and Yu, Stella X and Lin, Dahua},
  booktitle=CVPR,
  year={2018}
}

@inproceedings{gutmann2010noise,
  title={Noise-contrastive estimation: A new estimation principle for unnormalized statistical models},
  author={Gutmann, Michael and Hyv{\"a}rinen, Aapo},
  booktitle={AISTATS},
  year={2010},
  norganization={JMLR Workshop and Conference Proceedings}
}

@ARTICLE{Goodfellow13,
   author={Goodfellow, I.~J. and Mirza, M. and Xiao, D. and Courville, A. and Bengio, Y.},
    title="An Empirical Investigation of Catastrophic Forgetting in Gradient-Based Neural Networks",
  journal={arXiv preprint arXiv:1312.6211},
archivePrefix="arXiv",
   eprint={1312.6211},
 primaryClass="stat.ML",
 keywords={Statistics - Machine Learning, Computer Science - Learning, Computer Science - Neural and Evolutionary Computing, Empirical Study, Influential},
     year={2013},
    nmonth={dec},
   adsurl={http://adsabs.harvard.edu/abs/2013arXiv1312.6211G},
  adsnote={Provided by the SAO/NASA Astrophysics Data System},
  url={https://arxiv.org/abs/1312.6211},
}

@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proc. of the national academy of sciences},
  year={2017},
  publisher={National Acad Sciences},
    keywords={Regularization, Influential},
    url={https://www.pnas.org/content/pnas/114/13/3521.full.pdf},
}

@ARTICLE{Rusu16progressive,
   author={Rusu, A.~A. and Rabinowitz, N.~C. and Desjardins, G. and
	Soyer, H. and Kirkpatrick, J. and Kavukcuoglu, K. and
	Pascanu, R. and Hadsell, R.},
    title={Progressive Neural Networks},
  journal={arXiv 1606.04671},
archivePrefix="arXiv",
   eprint={1606.04671},
 primaryClass="cs.LG",
 keywords={Computer Science - Learning, Dynamic Architecture},
     year=2016,
    nmonth={jun},
   adsurl={http://adsabs.harvard.edu/abs/2016arXiv160604671R},
  adsnote={Provided by the SAO/NASA Astrophysics Data System},
   url={https://arxiv.org/abs/1606.04671}
}

@inproceedings{shin2017continual,
  title={Continual learning with deep generative replay},
  author={Shin, Hanul and Lee, Jung Kwon and Kim, Jaehong and Kim, Jiwon},
  booktitle=NIPS,
  year={2017},
}

@inproceedings{Lopez-Paz17,
title={Gradient Episodic Memory for Continual Learning},
author={Lopez-Paz, David and Ranzato, Marc-Aurelio},
booktitle=NIPS,
year={2017},
}

@inproceedings{Chaudhry19,
  title={Efficient Lifelong Learning with A-GEM},
  author={Chaudhry, Arslan and Ranzato, Marc’Aurelio and Rohrbach, Marcus and Elhoseiny, Mohamed},
  booktitle=ICLR,
  year={2019},
}

@article{serra2018overcoming,
  title=	 {Overcoming Catastrophic Forgetting with Hard Attention to the Task},
  author=	 {Serra, Joan and Suris, Didac and Miron, Marius and Karatzoglou, Alexandros},
  journal  ={ICML},
  year=	 {2018},
}

@inproceedings{chaudhry2018riemannian,
  title={Riemannian Walk for Incremental Learning: Understanding Forgetting and Intransigence},
  author={Chaudhry, Arslan and Dokania, Puneet K and Ajanthan, Thalaiyasingam and Torr, Philip HS},
  booktitle=ECCV,
  year={2018},
}

@inproceedings{Aljundi17,
  author   ={Rahaf Aljundi and Francesca Babiloni and Mohamed Elhoseiny and Marcus Rohrbach and Tinne Tuytelaars},
  title    ={Memory Aware Synapses: Learning what (not) to forget},
  booktitle=ECCV,
  year     ={2018},
}

@InProceedings{Zenke17,
  title=	 {Continual Learning Through Synaptic Intelligence},
  author=	 {Zenke, Friedeman and Poole, Ben and Ganguli, Surya },
  booktitle=	 {ICML},
  year=	 {2017},
}

@inproceedings{buzzega2020dark,
 author = {Buzzega, Pietro and Boschini, Matteo and Porrello, Angelo and Abati, Davide and Calderara, Simone},
 booktitle = NIPS,
 title = {Dark Experience for General Continual Learning: a Strong, Simple Baseline},
 year = {2020},
}

@inproceedings{fini2020online,
  title={Online Continual Learning under Extreme Memory Constraints},
  author={Fini, Enrico and Lathuilière, Stèphane and Sangineto, Enver and Nabi, Moin and Ricci, Elisa},
    booktitle=ECCV,
  year={2020},
}

@inproceedings{wu2019large,
  title={Large scale incremental learning},
  author={Wu, Yue and Chen, Yinpeng and Wang, Lijuan and Ye, Yuancheng and Liu, Zicheng and Guo, Yandong and Fu, Yun},
  booktitle=CVPR,
  year={2019},
}

@inproceedings{castro2018end,
  title={End-to-end incremental learning},
  author={Castro, Francisco M and Marin-Jimenez, Manuel J and Guil, Nicolas and Schmid, Cordelia and Alahari, Karteek},
  booktitle=ECCV,
  year={2018},
}

@inproceedings{rebuffi2017icarl,
  title={icarl: Incremental classifier and representation learning},
  author={Rebuffi, Sylvestre-Alvise and Kolesnikov, Alexander and Sperl, Georg and Lampert, Christoph H},
  booktitle=CVPR,
  year={2017},
}

@inproceedings{prabhu2020gdumb,
  title={GDumb: A simple approach that questions our progress in continual learning},
  author={Prabhu, Ameya and Torr, Philip HS and Dokania, Puneet K},
  booktitle=ECCV,
  pages={524--540},
  year={2020},
  organization={Springer},
  keywords={Empirical Study, Rehearsal}
}

@article{Robins95,
author = { Anthony   Robins },
title = {Catastrophic Forgetting, Rehearsal and Pseudorehearsal},
journal = {Connection Science},
year  = {1995},
}

@article{Li17learning,
  title={Learning without forgetting},
  author={Li, Zhizhong and Hoiem, Derek},
  journal=PAMI,
  year={2017},
}

@inproceedings{ostapenko2019learning,
  title={Learning to remember: A synaptic plasticity driven framework for continual learning},
  author={Ostapenko, Oleksiy and Puscas, Mihai and Klein, Tassilo and Jahnichen, Patrick and Nabi, Moin},
  booktitle=CVPR,
  year={2019},
}

@inproceedings{cha2021co2l,
  title={Co2l: Contrastive continual learning},
  author={Cha, Hyuntak and Lee, Jaeho and Shin, Jinwoo},
  booktitle=CVPR,
  pages={9516--9525},
  year={2021}
}


@article{oord2018representation,
  title={Representation learning with contrastive predictive coding},
  author={Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1807.03748},
  year={2018}
}

@article{tian2021divide,
  title={Divide and Contrast: Self-supervised Learning from Uncurated Data},
  author={Tian, Yonglong and Henaff, Olivier J and Oord, Aaron van den},
  journal={arXiv preprint arXiv:2105.08054},
  year={2021}
}

@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  journal={arXiv preprint arXiv:1503.02531},
  year={2015}
}

@inproceedings{tian2020contrastive,
  title={Contrastive multiview coding},
  author={Tian, Yonglong and Krishnan, Dilip and Isola, Phillip},
  booktitle=ECCV,
  pages={776--794},
  year={2020},
  organization={Springer}
}

@techreport{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex},
  year={2009},
  institution={Univ.\ Toronto},
}

@inproceedings{peng2019moment,
  title={Moment matching for multi-source domain adaptation},
  author={Peng, Xingchao and Bai, Qinxun and Xia, Xide and Huang, Zijun and Saenko, Kate and Wang, Bo},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle=CVPR,
  pages={770--778},
  year={2016}
}

@article{you2017large,
  title={Large batch training of convolutional networks},
  author={You, Yang and Gitman, Igor and Ginsburg, Boris},
  journal={arXiv preprint arXiv:1708.03888},
  year={2017}
}

@article{falcon2021aavae,
  title={AAVAE: Augmentation-Augmented Variational Autoencoders},
  author={Falcon, William and Jha, Ananya Harsh and Koker, Teddy and Cho, Kyunghyun},
  journal={arXiv preprint arXiv:2107.12329},
  year={2021}
}
@article{you2017large,
  title={Large batch training of convolutional networks},
  author={You, Yang and Gitman, Igor and Ginsburg, Boris},
  journal={arXiv preprint arXiv:1708.03888},
  year={2017}
}

@inproceedings{iscen2020memory,
  title={Memory-efficient incremental learning through feature adaptation},
  author={Iscen, Ahmet and Zhang, Jeffrey and Lazebnik, Svetlana and Schmid, Cordelia},
  booktitle={European Conference on Computer Vision},
  pages={699--715},
  year={2020},
  organization={Springer}
}

@article{rolnick2019experience,
  title={Experience replay for continual learning},
  author={Rolnick, David and Ahuja, Arun and Schwarz, Jonathan and Lillicrap, Timothy and Wayne, Gregory},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@inproceedings{fini2022self,
  title={Self-supervised models are continual learners},
  author={Fini, Enrico and da Costa, Victor G Turrisi and Alameda-Pineda, Xavier and Ricci, Elisa and Alahari, Karteek and Mairal, Julien},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9621--9630},
  year={2022}
}
